Impact of Log Parsing on Deep Learning-Based Anomaly Detection

Software systems log massive amounts of data, recording important runtime information. Such logs are used, for example, for log-based anomaly detection, which aims to automatically detect abnormal behaviors of the system under analysis by processing the information recorded in its logs. Many log-based anomaly detection techniques based on deep learning models include a pre-processing step called log parsing. However, understanding the impact of log parsing on the accuracy of anomaly detection techniques has received surprisingly little attention so far. Investigating what are the key properties log parsing techniques should ideally have to help anomaly detection is therefore warranted. In this paper, we report on a comprehensive empirical study on the impact of log parsing on anomaly detection accuracy, using 13 log parsing techniques, seven anomaly detection techniques (five based on deep learning and two based on traditional machine learning) on three publicly available log datasets. Our empirical results show that, despite what is widely assumed, there is no strong correlation between log parsing accuracy and anomaly detection accuracy, regardless of the metric used for measuring log parsing accuracy. Moreover, we experimentally confirm existing theoretical results showing that it is a property that we refer to as distinguishability in log parsing results as opposed to their accuracy that plays an essential role in achieving accurate anomaly detection.

==> tables/correlation_coefficient.tex <==
\pgfplotstabletypeset[
	col sep=comma,
	empty cells with={-}, %
	string replace={---}{\textemdash},
	every head row/.style={
		before row={\toprule
			\multicolumn{1}{c}{} & 
			\multicolumn{3}{c}{HDFS (reduced)} &
			\multicolumn{3}{c}{Hadoop}
			\\
			\cmidrule(r){2-4}
			\cmidrule(r){5-7}},
		after row=\midrule,
	},
	every last row/.style={after row=\bottomrule},
	every column/.style={fixed zerofill,precision=3},
	columns/AD_metric/.style={column type=l,column name=AD technique,string type},
	columns/HDFS_GA/.style={column type=r, column name=GA, precision=3},
	columns/HDFS_PA/.style={column type=r, column name=PA, precision=3},
	columns/HDFS_FTA/.style={column type=r, column name=FTA, precision=3, fixed},
	columns/Hadoop_GA/.style={column type=r, column name=GA, precision=3, fixed}, %fixed is used to remove exponent form
	columns/Hadoop_PA/.style={column type=r, column name=PA, precision=3, fixed},
	columns/Hadoop_FTA/.style={column type=r, column name=FTA, precision=3, fixed},
]{data/correlation_results.csv}


==> tables/datasets.tex <==
\begin{tabular}{l@{\hspace{2pt}}r@{\hspace{5pt}}r@{\hspace{5pt}}r@{\hspace{5pt}}r@{\hspace{5pt}}r@{\hspace{5pt}}r@{\hspace{5pt}}r@{\hspace{5pt}}}

\toprule
      Dataset & O & $L_{all}$ & $L_{n}$ & $L_{a}$ & $M_{all}$ & $M_{n}$ & $M_{a}$  \\
 \midrule
HDFS (reduced)  & 26 &  15295 & 15026 & 269 & 299971 & 292776 & 7195    \\
Hadoop &  175 & 54 & 11 & 43 & 109968 & 14392 & 95576  \\
OpenStack & 21 &  2068 & 2064  & 4 & 79925 & 79817 & 108   \\
\bottomrule
\end{tabular}




==> tables/datasets_literature.tex <==
%\begin{tabular}{l@{\hspace{2pt}}r@{\hspace{5pt}}}

%\toprule
%      Paper & Datasets  \\
% \midrule
%\cite{du2017deeplog}  & HDFS, OpenStack   \\
%\cite{zhang2019robust}  & HDFS, Proprietary Dataset   \\
%\cite{meng2019loganomaly}  & HDFS, BGL   \\
%\cite{xia2021loggan}  & HDFS, BGL   \\
%\cite{lu2018detecting}  & HDFS   \\
%\cite{hashemi2021detecting}  & HDFS   \\
%\cite{chen2021experience}  & HDFS, BGL   \\
%\cite{le2022log}  & HDFS, BGL, Spirit, Thunderbird   \\\
%\cite{le2021log}  & BGL, Thunderbird   \\
%\cite{fu2023empirical}  & HDFS, BGL, Thunderbird   \\
%\cite{huang2020hitanomaly} & HDFS, BGL, OpenStack \\
%\cite{qi2022adanomaly} & HDFS, BGL, OpenStack \\
%\bottomrule
%\end{tabular}




%\begin{tabular}{l@{\hspace{5pt}}r@{\hspace{5pt}}r@{\hspace{5pt}}r}
%
%\toprule
%      Datasets & Label & Code & Literature  \\
% \midrule
% 
% Android & \xmark &  \xmark & - \\
% Apache & \xmark &  \xmark & -  \\
% BGL & \cmark & \xmark & \cite{meng2019loganomaly,xia2021loggan,chen2021experience,le2022log,
% le2021log,fu2023empirical,huang2020hitanomaly,qi2022adanomaly}\\
% HDFS &  \cmark &  \cmark & \cite{du2017deeplog,zhang2019robust,meng2019loganomaly,
% xia2021loggan,hashemi2021detecting,chen2021experience,le2022log,fu2023empirical,
% huang2020hitanomaly,qi2022adanomaly} \\
% HPC & \xmark &  \xmark & -  \\
% Hadoop &  \cmark & \cmark& - \\
% HealthApp & \xmark &  \xmark &-   \\
% Linux & \xmark &  \xmark & -  \\
% Mac & \xmark & \xmark &  - \\
% OpenSSH & \xmark & \xmark & -  \\
% OpenStack &  \cmark &  \cmark & \cite{du2017deeplog,huang2020hitanomaly,qi2022adanomaly}  \\
% Proxifier & \xmark &  \xmark & -  \\
% Spark & \xmark & \xmark & -  \\
% Spirit & \cmark & \xmark & \cite{le2022log}  \\
% Thunderbird & \cmark & \xmark & \cite{le2022log,le2021log,fu2023empirical}   \\
% Windows & \xmark &  \xmark & -   \\
% Zookeeper & \xmark &  \xmark & -  \\
% 
%\bottomrule
%\end{tabular}


\begin{tabular}{lrr}

\toprule
      Datasets & Anomaly Label & Source Code  \\
 \midrule
 
 Android & \xmark &  \xmark \\
  Apache & \xmark &  \xmark  \\
   BGL & \cmark & \xmark \\
   \rowcolor{lightgray}
 HDFS &  \cmark &  \cmark  \\
  HPC & \xmark &  \xmark  \\
   \rowcolor{lightgray}
 Hadoop &  \cmark & \cmark \\
 HealthApp & \xmark &  \xmark  \\
 Linux & \xmark &  \xmark \\
 Mac & \xmark & \xmark \\
  OpenSSH & \xmark & \xmark  \\
   \rowcolor{lightgray}
 OpenStack &  \cmark &  \cmark   \\
 Proxifier & \xmark &  \xmark  \\
 Spark & \xmark & \xmark  \\
 Spirit & \cmark & \xmark  \\
 Thunderbird & \cmark & \xmark    \\
 Windows & \xmark &  \xmark \\
 Zookeeper & \xmark &  \xmark \\
 
\bottomrule
\end{tabular}



%\begin{tabular}{l@{\hspace{5pt}}r@{\hspace{5pt}}r@{\hspace{5pt}}}
%\toprule
 %     Datasets & Labelled Information  & Source Code Availability \\
 %\midrule
 
% HDFS &  \cmark &  \cmark  \\
% Hadoop &  \cmark & \cmark \\
% OpenStack &  \cmark &  \cmark  \\
% BGL & \xmark & \xmark \\
 %Thunderbird & \xmark & \xmark    \\
 %Spirit & \xmark & \xmark   \\
 
%\bottomrule
%\end{tabular}


%%% Local Variables:
%%% mode: latex
%%% TeX-master: "../main"
%%% End:


==> tables/hadoop_rq2.tex <==
\pgfplotstabletypeset[
	col sep=comma,
	fixed zerofill, fixed,
	precision=3,
	every head row/.style={
		before row={
	   		\toprule
			\multicolumn{1}{c}{} & 
			\multicolumn{3}{c}{DeepLog (F1)} &
			\multicolumn{3}{c}{LogAnomaly (F1)} &
			\multicolumn{3}{c}{LogRobust (F1)} &
			\multicolumn{3}{c}{CNN (F1)} &
			\multicolumn{3}{c}{PLELog (F1)} 
			\\
			\cmidrule(r){2-4}
			\cmidrule(r){5-7}
			\cmidrule(r){8-10}
			\cmidrule(r){11-13}
			\cmidrule(r){14-16}
		},
		after row=\midrule,
	},
	every last row/.style={
		before row=\midrule,
		after row=\bottomrule,
	},
	columns/TI/.style={column type=l,column name=Log Parser, string type },
	columns/AD_DeepLog_F1_dist/.style={column type=r,column name=$R_\mathit{dst}$},
	columns/AD_DeepLog_F1_indist/.style={column type=r, column name=$R_\mathit{ind}$},
	columns/DeepLog_delta/.style={column type=r, column name=$\Delta$},
	columns/AD_LogAnomaly_F1_dist/.style={column type=r,column name=$R_\mathit{dst}$},
	columns/AD_LogAnomaly_F1_indist/.style={column type=r, column name=$R_\mathit{ind}$},
	columns/LogAnomaly_delta/.style={column type=r, column name=$\Delta$},
	columns/AD_LogRobust_F1_dist/.style={column type=r,column name=$R_\mathit{dst}$},
	columns/AD_LogRobust_F1_indist/.style={column type=r, column name=$R_\mathit{ind}$},
	columns/LogRobust_delta/.style={column type=r, column name=$\Delta$},
	columns/AD_CNN_F1_dist/.style={column type=r,column name=$R_\mathit{dst}$},
	columns/AD_CNN_F1_indist/.style={column type=r,column name=$R_\mathit{ind}$},
	columns/CNN_delta/.style={column type=r, column name=$\Delta$},
	columns/AD_PLELog_F1_dist/.style={column type=r,column name=$R_\mathit{dst}$},
	columns/AD_PLELog_F1_indist/.style={column type=r,column name=$R_\mathit{ind}$},
	columns/PLELog_delta/.style={column type=r, column name=$\Delta$}
]{data/Hadoop_RQ2.csv}


==> tables/hadoop_rq2_ml.tex <==
\pgfplotstabletypeset[
	col sep=comma,
	fixed zerofill, fixed,
	precision=3,
	every head row/.style={
		before row={
	   		\toprule
			\multicolumn{1}{c}{} & 
			\multicolumn{3}{c}{SVM (F1)} &
			\multicolumn{3}{c}{RF (F1)} 
			\\
			\cmidrule(r){2-4}
			\cmidrule(r){5-7}
		},
		after row=\midrule,
	},
	every last row/.style={
		before row=\midrule,
		after row=\bottomrule,
	},
	columns/TI/.style={column type=l,column name=Log Parser, string type },
			columns/AD_SVM_F1_dist/.style={column type=r,column name=$R_\mathit{dst}$},
	columns/AD_SVM_F1_indist/.style={column type=r,column name=$R_\mathit{ind}$},
	columns/SVM_delta/.style={column type=r, column name=$\Delta$},
		columns/AD_RF_F1_dist/.style={column type=r,column name=$R_\mathit{dst}$},
	columns/AD_RF_F1_indist/.style={column type=r,column name=$R_\mathit{ind}$},
	columns/RF_delta/.style={column type=r, column name=$\Delta$},
]{data/Hadoop_RQ2_ML.csv}


==> tables/hdfs_rq2.tex <==
\pgfplotstabletypeset[
	col sep=comma,
	fixed, fixed zerofill,
	empty cells with={-}, % to insert a hyphen in empty cells automatically
	precision=3,
	every head row/.style={
		before row={
	   		\toprule
			\multicolumn{1}{c}{} & 
			\multicolumn{3}{c}{DeepLog (F1)} &
			\multicolumn{3}{c}{LogAnomaly (F1)} &
			\multicolumn{3}{c}{LogRobust (F1)} &
			\multicolumn{3}{c}{CNN (F1)} &
			\multicolumn{3}{c}{PLELog (F1)} 
			\\
			\cmidrule(r){2-4}
			\cmidrule(r){5-7}
			\cmidrule(r){8-10}
			\cmidrule(r){11-13}
			\cmidrule(r){14-16}
		},
		after row=\midrule,
	},
	every last row/.style={
		before row=\midrule,
		after row=\bottomrule,
	},
	columns/TI/.style={column type=l,column name=Log Parser,string type},
	columns/AD_DeepLog_F1_dist/.style={column type=r,column name=$R_\mathit{dst}$},
	columns/AD_DeepLog_F1_indist/.style={column type=r, column name=$R_\mathit{ind}$},
	columns/DeepLog_delta/.style={column type=r, column name=$\Delta$},
	columns/AD_LogAnomaly_F1_dist/.style={column type=r,column name=$R_\mathit{dst}$},
	columns/AD_LogAnomaly_F1_indist/.style={column type=r, column name=$R_\mathit{ind}$},
	columns/LogAnomaly_delta/.style={column type=r, column name=$\Delta$},
	columns/AD_LogRobust_F1_dist/.style={column type=r,column name=$R_\mathit{dst}$},
	columns/AD_LogRobust_F1_indist/.style={column type=r, column name=$R_\mathit{ind}$},
	columns/LogRobust_delta/.style={column type=r, column name=$\Delta$},
	columns/AD_CNN_F1_dist/.style={column type=r,column name=$R_\mathit{dst}$},
	columns/AD_CNN_F1_indist/.style={column type=r,column name=$R_\mathit{ind}$},
	columns/CNN_delta/.style={column type=r, column name=$\Delta$},
	columns/AD_PLELog_F1_dist/.style={column type=r,column name=$R_\mathit{dst}$},
	columns/AD_PLELog_F1_indist/.style={column type=r,column name=$R_\mathit{ind}$},
	columns/PLELog_delta/.style={column type=r, column name=$\Delta$}
]{data/HDFS_RQ2.csv}


==> tables/hdfs_rq2_ml.tex <==
\pgfplotstabletypeset[
	col sep=comma,
	fixed, fixed zerofill,
	empty cells with={-}, % to insert a hyphen in empty cells automatically
	precision=3,
	every head row/.style={
		before row={
	   		\toprule
			\multicolumn{1}{c}{} & 
			\multicolumn{3}{c}{SVM (F1)} &
			\multicolumn{3}{c}{RF (F1)} 
			\\
			\cmidrule(r){2-4}
			\cmidrule(r){5-7}
		},
		after row=\midrule,
	},
	every last row/.style={
		before row=\midrule,
		after row=\bottomrule,
	},
	columns/TI/.style={column type=l,column name=Log Parser,string type},
		columns/AD_SVM_F1_dist/.style={column type=r,column name=$R_\mathit{dst}$},
	columns/AD_SVM_F1_indist/.style={column type=r,column name=$R_\mathit{ind}$},
	columns/SVM_delta/.style={column type=r, column name=$\Delta$},
		columns/AD_RF_F1_dist/.style={column type=r,column name=$R_\mathit{dst}$},
	columns/AD_RF_F1_indist/.style={column type=r,column name=$R_\mathit{ind}$},
	columns/RF_delta/.style={column type=r, column name=$\Delta$},
]{data/HDFS_RQ2_ML.csv}


==> tables/related_work_comparison.tex <==
\begin{tabularx}{\linewidth}{XXXX}
\toprule
      Category & \citet{le2022log} & \citet{fu2023empirical} & Our work   \\
 \midrule
 \rowcolor{gray!25}
Objective & Investigate different factors that might affect anomaly detection accuracy & 
Investigate the impact of log parsing techniques on anomaly detection accuracy & 
Evaluate the impact of log parsing accuracy and the distinguishability of log parsing results on anomaly detection accuracy \\ 
Log parsing accuracy metrics & N/A &PA &  PA, GA, and TA     \\
 \rowcolor{gray!25}
Oracle templates & N/A & Manually generated for 2K sample log messages & Extracted from the corresponding source code \\
Logs used for measuring log parsing accuracy & N/A & Only a small fraction of logs actually used for anomaly detection & All logs used for anomaly detection \\
 \rowcolor{gray!25}
Log parsing techniques & Drain, Spell, IPLoM and AEL & Drain, Spell, IPLoM, LFA, Logram, and LenMa  & Drain, Spell, IPLoM, AEL, LFA, Logram, LenMa, LogSig, LogCluster, LogMine, SHISO, MoLFI, and SLCT\\
Anomaly detection techniques & DeepLog, LogRobust, LogAnomaly, PLELog, and CNN & DeepLog, LogRobust, Principal Component Analysis (PCA), LogClustering, Logistic Regression (LR), and Decision Tree (DT) & DeepLog, LogRobust, LogAnomaly, PLELog, CNN, \rev{SVM, and RF}   \\
 \rowcolor{gray!25}
Distinguishability~\cite{shin2021theoretical} & Not considered & Not considered & Considered \\


\bottomrule
\end{tabularx}


